Quantifying Spatial Audio Quality Impairment

Spatial audio quality is a highly multifaceted concept, with many interactions between environmental, geometrical, anatomical, psychological, and contextual considerations. Methods for characterization or evaluation of the geometrical components of spatial audio quality, however, remain scarce, despite being perhaps the least subjective aspect of spatial audio quality to quantify. By considering interchannel time and level differences relative to a reference signal, it is possible to construct a signal model to isolate some of the spatial distortion. By using a combination of least-square optimization and heuristics, we propose a signal decomposition method to isolate the spatial error from a processed signal, in terms of interchannel gain leakages and changes in relative delays. This allows the computation of simple energy-ratio metrics, providing objective measures of spatial and non-spatial signal qualities, with minimal assumptions and no dataset dependency. Experiments demonstrate the robustness of the method against common spatial signal degradation introduced by, e.g., audio compression and music source separation. Implementation is available at https://github.com/karnwatcharasupat/spauq.

==> abbrev.tex <==

\DefineSpuriousJournalWord{The}

\DefineJournalAbbreviation{Transactions}{Trans}

% %%%%%%%%%%%% Audio Journal %%%%%%%%%%%%

% % TASLP
% \DefineJournalException{IEEE/ACM Transactions on Audio Speech and Language Processing}{IEEE/ACM Trans. ASLP}
% \DefineJournalException{IEEE Transactions on Audio Speech and Language Processing}{IEEE Trans. ASLP}

% \DefineJournalException{Journal of the Acoustical Society of America}{J. ASA}
% \DefineJournalException{The Journal of the Acoustical Society of America}{J. ASA}

% %%%%%%%%%%%% Audio Conf %%%%%%%%%%%%

% % ICASSP
% \DefineJournalException{Proceedings of the IEEE International Conference on Acoustics, Speech and Signal Processing}{ICASSP}
% \DefineJournalException{Proceedings of the 2022 IEEE International Conference on Acoustics, Speech and Signal Processing}{ICASSP}
% \DefineJournalException{Proceedings of the 2017 IEEE International Conference on Acoustics, Speech and Signal Processing}{ICASSP}

% % Interspeech
% \DefineJournalException{Proceedings of the Annual Conference of the International Speech Communication Association}{Interspeech}

% % Internoise
% \DefineJournalException{Proceedings of the 45th International Congress and Exposition on Noise Control Engineering}{Internoise}
% \DefineJournalException{Proceedings of the 46th International Congress and Exposition on Noise Control Engineering}{Internoise}
% \DefineJournalException{Proceedings of the 49th International Congress and Expo on Noise Control Engineering}{Internoise}
% \DefineJournalException{Proceedings of the 51st International Congress and Expo on Noise Control Engineering}{Internoise}

% % ICA
% \DefineJournalException{Proceedings of the International Congress on Acoustics}{ICA}

% %%%%%%%%%%%% AI Conf %%%%%%%%%%%%

% % EMNLP
% \DefineJournalException{Proceedings of the Conference on Empirical Methods in Natural Language Processing}{EMNLP}

% % CVPR
% \DefineJournalException{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}{CVPR}

% % ICLR
% \DefineJournalException{Proceedings of the 3rd International Conference on Learning Representations}{ICLR}
% \DefineJournalException{Proceedings of the 6th International Conference on Learning Representations}{ICLR}

% % NeurIPS
% \DefineJournalException{Proceedings of the Conference on Neural Information Processing Systems}{NeurIPS}

% % ICML
% \DefineJournalException{Proceedings of the 38th International Conference on Machine Learning}{ICML}

% % AAAI
% \DefineJournalException{Proceedings of the 34th AAAI Conference on Artificial Intelligence}{AAAI}

==> tables/bss.tex <==
\begin{table*}[h]
    \centering
    \caption{Music BSS Benchmark}
    \begin{tabularx}{\linewidth}{ll@{ }rrrrrrrr}
        \toprule
        Model & Variant && IDR & IFR & ISR & SRR & SDR & SIR & SAR   \\
        \midrule
        Oracle \\
        % FastICA & & \cite{Hyvarinen2000IndependentApplications}\\
        Open-Unmix
            & \texttt{umxl} & \cite{Stoter2019Open-UnmixSeparation}\\
            & \texttt{umx} & \cite{Stoter2019Open-UnmixSeparation}\\
        Demucs & v3 & \cite{Defossez2021HybridSeparation}\\
                & v4 & \cite{Rouard2022HybridSeparation} \\
        Spleeter & 4 stems& \cite{Hennequin2020Spleeter:Models} \\
        \bottomrule
    \end{tabularx}
    \label{tab:my_label}
\end{table*}

==> tables/codec.tex <==
\begin{table}[t]
    \centering
    \caption{Compression Benchmark}
    \begin{tabularx}{\linewidth}{lllrrrrr}
        \toprule
        Dataset & Algo & Bitrate & Coding Mode & IDR & ISR & SRR & SNR   \\
        \midrule
        TIMIT & MP3 & \\
        & Opus & \\
        \midrule
        MUSDB & MP3 & \\
        & Opus & \\
        \midrule
        EBU & MP3 & \\
        & Opus & \\
        \bottomrule
    \end{tabularx}
    \label{tab:my_label}
\end{table}
